A Deterministic Distributed Algorithm for Exact Weighted All-Pairs Shortest Paths in $\tilde{O}(n^{3/2})$ Rounds

We present a deterministic distributed algorithm to compute all-pairs shortest paths(APSP) in an edge-weighted directed or undirected graph. Our algorithm runs in $\tilde{O}(n^{3/2})$ rounds in the Congest model, where $n$ is the number of nodes in the graph. This is the first $o(n^2)$ rounds deterministic distributed algorithm for the weighted APSP problem. Our algorithm is fairly simple and incorporates a deterministic distributed algorithm we develop for computing a `blocker set' \cite{King99}, which has been used earlier in sequential dynamic computation of APSP.

==> centers.tex <==
\section{Deterministic Weighted APSP in $\tilde{O}(n^{3/2})$ or Less}\label{sec:outline}

 We describe a simple deterministic weighted APSP algorithm in the \congest model that runs in $O(n^{3/2})$ rounds.
 The algorithm is also a template for  computing APSP deterministically with even a smaller number of rounds if 
 $h$-APSP can be computed in a smaller number of rounds. Very recently such an algorithm was designed in~\cite{AR18b},
 and we discuss the impact of that algorithm at the end of the paper.
 
 
 Let the edge-weighted input graph be $G=(V,E)$ with weight function $w$ and with $|V|=n$ and $|E|=m$. The \congest{} model assumes that every message is of $O(\log n)$-bit size, which restricts $w(e)$ to be an $O(\log n)$ size integer value. However,
 outside of this restriction imposed by the \congest model, our algorithm works for arbitrary edge-weights (even negative edge-weights as long as there is no negative-weight cycle).
 
 
 Our overall APSP algorithm is given in Algorithm~\ref{alg6}.
  We first observe that and $h$-hop SSSP tree rooted at a vertex $s$ can be computed in $O(h)$ rounds by running the
  Bellman-Ford algorithm for $h$ rounds. 
  %We fix a value for $h$ ($h= \sqrt n$ gives our $O(\n^{3/2})$-round algorithm).
  Using Bellman-Ford, our algorithm first computes an $h$-hop SSSP tree for each vertex $v$ in $O(n \cdot h)$ rounds.
  It then finds a collection of $b=O(n/h)$  nodes called {\it centers} (or {\it distinguished nodes}~\cite{UY91} or {\it centers}~\cite{HNS17})
  such that there is a center node in any subpath of length $h$ in every $h$-hop shortest path tree we have computed.
  Once we have our center set we can compute APSP  by first computing SSSP for each center (using
  the Bellman-Ford algorithm) and then broadcasting each node's shortest path distances from each of the $b$ centers
  to all other nodes; both of these steps are readily performed in $O(n\cdot b)$ rounds. When $h = \sqrt n$ the number of centers 
  is also $O(\sqrt n)$ hence the overall algorithm runs in $O(n^{3/2}$) rounds provided we can find the desired centers 
  efficiently and deterministically. 
  
  \begin{algorithm}[H]	
%\scriptsize
\caption{ Main Algorithm}
\begin{algorithmic}[1]	
\State Compute an $h$-hop SSSP tree for each $v\in V$.  \label{alg6:h-hop-sssp-tree}
% (If $h= \tilde{O}(\sqrt n)$ run Bellman-Ford for $h$ rounds from each source.)
\State  Compute  $\tilde{O}(n/h)$ centers and store in $\ce$ using Algorithm~\ref{alg5}.
\State {\bf for each} $c\in \ce$ in sequence: send $\delta(v,c)$ value to each $v$ whose $h$-hop tree contains $c$. \label{alg6:center-to-h-hop-root}
\State  {\bf for each} $c \in \ce$  in sequence: run Bellman-Ford from $c$ to compute $\delta (c,v)$ at each $v \in V$.	\label{alg6:bf}
\State {\bf for each} $c \in \ce$ in sequence:  broadcast from each $v\in V$ its $\delta(c,v)$ value to all other nodes.	\label{alg6:broadcast}
\State {\bf Local step at each node:} At each $v$ compute $\delta(u,v)$ values for each $u \in V$ by using the $h$-hop  $\delta(v,c)$ values at $v$ received in 
Step~\ref{alg6:center-to-h-hop-root}  and the $\delta (c,u)$ values for all $c\in \ce$ received in Step~\ref{alg6:broadcast}.
\end{algorithmic} \label{alg6}
\end{algorithm}

  
  \subsection{Finding Centers for a Collection of $h$-hop Trees}\label{sec:blockers-outline}
  
  The simplest method to find a set of centers is to chose them randomly. This method was first used by
  Ullman and Yannakakis where they picked a random set of $O(\sqrt n \cdot \log n)$ centers (or distinguished nodes)
  which are readily seen to intersect any path of $O(\sqrt n)$ vertices. Using this set they computed the transitive closure
  (and some single source problems) more efficiently in parallel (in the PRAM model) in $O(n^{\epsilon})$ time than
  the matrix-multiplication based method. This method of choosing suitable centers has been used extensively in parallel and dynamic computation of transitive closure and shortest paths, and more recently, has been used in distributed 
  computation of APSP~\cite{HNS17}.
  
  In order to compute
  fully-dynamic APSP, King~\cite{King99} gave a deterministic sequential algorithm to compute a blocker set in the 
  following setting.
  
  
  A deterministic sequential algorithm for computing blockers was given in~\cite{King99} in order to compute
  fully dynamic APSP. We now briefly describe the results in~\cite{King99} that we will use in our distributed algorithm
  for computing a set of $O(n/h)$ centers. 
  
  
  \begin{definition}[(\cite{King99})]
  Let $F$ be a collection of  $h$-hop SSSP trees for the graph $G=(V,E)$. A set $B \subset V$ is a \emph{blocker} for $F$
  if every path from the root of a tree to a descendant leaf contains a vertex in $B$.
  \hide{
  $S$ is a blocker set for $F$ if for each pair of vertices $s, t \in V$ such that 
the shortest path from $s$ to $t$ has more than $h$ hops,
then there exists vertices $c_1, c_2,\ldots, c_l \in S$ where $l > 0$ 
such that the shortest path can be represented as 
$(s,c_1) \circ (c_1,c_2) \circ \ldots \circ (c_{l-1},c_l) \circ (c_l,t)$,
where $(c_i,c_{i+1})$ refers to the shortest path from $c_i$ to $c_{i+1}$
and each of these paths have hop-length at most $h$.
}% end hide
\end{definition}

A deterministic algorithm that computes a blocker set of size $O((n/h) \log n)$ in $O(n^2 + nh \log n)$ time is given in~\cite{King99}.
It uses the observation that, given the collection of trees $F$ with totally $p$ leaves across all trees (and hence $p$ root to leaf
paths), there must exist a vertex that is contained in at least
$ph/n$. The algorithm add one such vertex to the blocker set,
removes all paths that are covered by this vertex and repeats this process until no path remains. The number of paths is
reduced from $p$ to at most $(1-h/n) \cdot p$ when the blocker vertex is removed, hence after $O((n/h) \ln p)$ removals of
vertices, all paths are removed. The result follows since $p$ is at most $n^2$.

We now give a deterministic distributed algorithm to compute a set of $b= O((n/h) \log n)$ centers in $O(n \cdot b)$ rounds
given the collection $F$ of $h$-hop SSSP trees for every source $s\in V$. We assume that for s tree $T_s$ rooted at
$s$, each node $v$ in the tree knows $\delta(s,v)$, its shortest path distance from $s$, its hop length $h_{s}(v)$ (the
number of edges on the tree path from $s$ to $v$, and the identities of its parent node and its children in $T_s$.
Initially our algorithm will compute, for each node $v$, the values  $score_s(v)$ for each root $s$, which is the number of leaves in
the subtree rooted at $v$ in the tree with root $s$, and $score(v)$, which is the sum of the $n$ $score_s(v)$ values.
These
values are computed in Algorithm~\ref{alg4}
are readily computed in $O(h)$ rounds per tree by running the Bellman-Ford algorithm `in reverse' (this is a simple 
method developed in~\cite{PR18} to compute betweenness centrality values after the computation of APSP).  The
method works as follows.
 Let
us assume that the $h$-hop SSSP trees for the $n$ sources were computed by an Algorithm $h$-Hop, where each vertex
$v$ can identify a round number $r_x$ in which it sent out its finalized SSSP distance from source $s$. Clearly these
round numbers will be different for different sources. Algorithm~\ref{alg4}, the $score_x(v)$ values are propagated from
the leaves of each tree towards the root by running the rounds of Algorithm $h$-Hop in reverse. Hence, if $v$ sent out
its SSSP distance for source $x$ to its children in round $r$ of Algorithm $h$-Hop and if Algorithm $h$-hop took $R$
rounds in total, then $v$ will sent out its score$x_(v)$ value to its parent in round $R-r$ of Algorithm~\ref{alg4}. It is
readily verified by induction that $v$'s children would have sent their scores to $v$ in an earlier round than $R-r$ since
none of $v$'s children could have sent out their finalized value in a round before $r$.

\begin{algorithm}[H]	
%\scriptsize
\caption{Initialize scores each node for all $h$-hop trees }
\begin{algorithmic}[1]	
\State Run an $h$-hop APSP algorithm and store at $v$ the round $r_{x}(v)$ in which $\delta(x,v)$ was sent out by $v$ to its children.  Let $R$ denote the total number of rounds used by Algorithm $h$-hop APSP.
\State {\bf for each} node $v$ and each root $x$ {\bf if} $l_x (v) = h$ {\bf then} $score_x (v) \leftarrow 1$ {\bf else} $score_x(v) \leftarrow 0$
\State {\bf In round $r > 0$:}
\State {\bf send:} {\bf for  each} $v \in V$  {\bf if} $r = R - r_{x}(v)$ for some $x$ {\bf then} send $\langle score_x (v), x \rangle$ to $parent_x(v)$ 	\label{alg3:sendStart}
%	\EndFor		\label{alg3:sendEnd}
\State {\bf receive [lines~\ref{alg3:newreceiveStart}-\ref{alg3:receiveEnd}]:}   for each $v\in V$ let $\mathcal{I}_v$ be the set of incoming messages to $v$ \label{alg3:newreceiveStart}
\State $~~$ {\bf for each} $M \in \mathcal{I}_v$ \label{alg3:receiveStart}
	\State $~~$ let $M = \langle score^-, x \rangle$ and let the sender be $w$
	 \State $~~$ {\bf if} $w$ is a child of $v$ in $t_x$ {\bf then} $score_x (v) \leftarrow score_x (v) + score^-$  \label{alg3:receiveEnd}
%	\EndFor \label{alg3:receiveEnd}
\end{algorithmic} \label{alg3}
\end{algorithm}

\begin{algorithm}[H]	
%\scriptsize
\caption{ Update scores at node $v$ after center $c$ is selected}
Input: center $c$, collection of  already selected centers $\mathcal{C}$
\begin{algorithmic}[1]	
\State {\bf Initialization [lines~\ref{alg4:initStart}-\ref{alg4:initEnd}]:}
\If{$c = v$}	\label{alg4:initStart}
	\For{each $x \in S$}
		\If{$score_x (v) \neq 0$}
			\State add an entry $Z = \langle x, score_x (v) \rangle$ to $list_v^{anc}$; $sent(Z) \leftarrow false$
			\State add an entry $Z = \langle x \rangle$  to $list_v^{des}$; $sent(Z) \leftarrow false$
			\State $\sxv \leftarrow 0$
		\EndIf
	\EndFor
	\State $\sv \la 0$
\EndIf	\label{alg4:initEnd}
\State {\bf In round $r > 0$: (only for vertices in $v \in V - \mathcal{C} \cup \{c\}$)} \vspace{0.05in}
\State {\bf send [lines~\ref{alg4:sendStart}-\ref{alg4:sendEnd}]:}
\State Let $Z_1 = \langle x \rangle$ be the unsent entry with the smallest ID in \lvd	\label{alg4:sendStart}
% \State $M_1 \leftarrow \langle Z_1 \rangle$
\State send $\langle Z_1\rangle$ to all descendants of $v$ in $x$'s tree; $sent(Z_1) \leftarrow true$
\State Let $Z_2 = \langle x, \sxv \rangle$  be the corresponding entry in \lva
% \State $M_2 \leftarrow \langle Z_2 \rangle$
\If{$v \neq x$}
	\State send $\langle Z_2\rangle$ to $v$'s parent in $x$'s tree; $sent(Z_2) \leftarrow true$ \vspace{0.05in}
\EndIf	\label{alg4:sendEnd}
\State {\bf receive [lines~\ref{alg4:receiveStart}-\ref{alg4:receiveEnd}]:}
\State Let $\mathcal{I}$ be the set of incoming messages	\label{alg4:receiveStart}
\For{{\bf each} $M \in \mathcal{I}$}
%	\State let $Z$ be the entry in $M$.
	\If{$M$ is of the form $\langle x \rangle$}
		\State $\sxv \leftarrow 0$;  $\sv \leftarrow \sv - \sxv$; add $Z$ to \lvd
	\Else ($M$ is of the form $\langle x, \s \rangle$)
		\State $\sxv \leftarrow \sxv - \s$;  $\sv \leftarrow \sv - \s$; add $Z$ to \lva
	\EndIf
\EndFor	\label{alg4:receiveEnd}
\end{algorithmic} \label{alg4}
\end{algorithm}

\begin{algorithm}[H]	
%\scriptsize
\caption{Algorithm for computing centers at node $v \in V$ }
\begin{algorithmic}[1]	
\State Run Algorithm~\ref{alg3} to compute scores 
\State $score(v) \leftarrow 0$ 
\State {\bf for each} $x \in S$ $score(v) \leftarrow score(v) + score_x (v)$ 
\State broadcast $\sv$ to all nodes in $V$
\State {\bf while} there is a node $c$ with $score (c) > 0$
\State \hspace{.5in} let $c$ be the node with max score
\State  \hspace{.5in} Run Algorithm~\ref{alg4} to update $\sxv$ for each $x \in S$ and $\sv$
\State \hspace{.5in} broadcast $\sv$ to all nodes in $V$
\end{algorithmic} \label{alg5}
\end{algorithm}

\begin{lemma}
Let $c$ be the new chosen center.
Then Algorithm~\ref{alg4} correctly updates the value of  $\sxv$ for each source $x \in S$ and
 node $v \notin \mathcal{C}$.
\end{lemma}


\bl
For each node $v \in V$,
Algorithm~\ref{alg6} correctly computes the shortest path distance values from each $s \in V$ to $v$ in
$\tilde{O} (R(h) + n\cdot \frac{n}{h})$,
where $R(h)$ denotes the number of rounds required to compute $h$ hop APSP.
\el

\begin{proof}
Algorithm~\ref{alg5} correctly computes $h$ hop APSP
and the set $\ce$ in $\tilde{O} (R(h) + n\cdot \frac{n}{h})$ rounds.
Since there are $\tilde{O}(\frac{n}{h})$ centers, 
all the Bellman Ford executions in Step~\ref{alg6:bf} can be finished in $\tilde{O}(n\cdot \frac{n}{h})$ rounds.
In Step~\ref{alg6:broadcast},
each node $v$ needs to broadcast $\tilde{O}(\frac{n}{h})$ values,
thus the congestion at any node is bounded by $\tilde{O}(n\cdot \frac{n}{h})$,
and hence all the nodes receive all the broadcasted values by $\tilde{O}(n\cdot \frac{n}{h})$ rounds.
\end{proof}
